Zero-Shot Visualization: Exploring Text Corpora with User-Prompted Axes

We study the application of large language models (LLMs) to the visual exploration of textual corpora. We introduce zero-shot visualization (ZSV), a task in which users specify concepts in natural language and documents are mapped onto the corresponding concept axes for visualization. Building a ZSV system of practical value is non-trivial, as it requires choices at the intersection of feature functions, efficient implementation tradeoffs, and pre/post-processing decisions affecting visualization quality. To that end, we establish a benchmark that compares methods spanning embedding similarity, direct semantic judgments, and conditional likelihood estimation in this setting. Across multiple datasets and use cases we evaluate the properties of different scoring methods and design choices in terms of semantic faithfulness, score fidelity, and computational cost. Our results identify that scoring based on next-token probabilities offers the strongest practical trade-off among the evaluated methods. We further apply this approach to unlabeled corpora to examine its behavior in realistic exploratory settings. These experiments highlight additional design considerations, including the use of graded axes together with binary relevance filtering, and reveal a compositional sentiment bias in off-topic documents. Based on these findings, we provide practical guidelines for constructing end-to-end ZSV baselines.

==> figures/fig_hotel_2x2.tex <==
\usetikzlibrary{matrix,positioning}

\begin{figure}[!t]
\centering
\footnotesize

\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.0}

\begin{tabular}{c c c}

% -------- Column titles --------
&
\multicolumn{1}{c}{\textbf{Retriever-based scorers}}
&
\multicolumn{1}{c}{\textbf{LLM-based scorers}}
\\[6pt]

% -------- Row 1 --------
\parbox[c][0.55\linewidth][t]{1.8em}{%
  \vspace*{2cm}
  \rotatebox{90}{Does the review talk about hotel staff?}
}
&
\begin{subfigure}[t]{0.44\linewidth}
  \centering
  \includegraphics[width=\linewidth, trim={6pt 6pt 6pt 6pt},clip]{figures/hotel_tfidf.pdf}
  \caption{Sparse Lexical}
\end{subfigure}
&
\begin{subfigure}[t]{0.44\linewidth}
  \centering
  \includegraphics[width=\linewidth, trim={6pt 6pt 6pt 6pt},clip]{figures/hotel_direct_rating.pdf}
  \caption{Direct Rating}
\end{subfigure}
\\[-40pt]

% -------- Row 2 --------
&
\begin{subfigure}[t]{0.44\linewidth}
  \centering
  \includegraphics[width=\linewidth, trim={6pt 6pt 6pt 6pt},clip]{figures/hotel_cosine.pdf}
  \caption{Dense Neural}
\end{subfigure}
&
\begin{subfigure}[t]{0.44\linewidth}
  \centering
  \includegraphics[width=\linewidth, trim={6pt 6pt 6pt 6pt},clip]{figures/hotel_zero_shot.pdf}
  \caption{Prob.\ Zero-Shot}
\end{subfigure}
\\[20pt]

% -------- Row 3 --------
&
\begin{subfigure}[t]{0.44\linewidth}
  \centering
  \includegraphics[width=\linewidth, trim={6pt 6pt 6pt 6pt},clip]{figures/hotel_neural_sparse_retriever.pdf}
  \caption{Sparse Neural}
\end{subfigure}
&
\begin{subfigure}[t]{0.44\linewidth}
  \centering
  \includegraphics[width=\linewidth, trim={6pt 6pt 6pt 6pt},clip]{figures/hotel_explanation_marginalized.pdf}
  \caption{Expl.-Marg.}
\end{subfigure}
\\[20pt]

% -------- X-axis label --------
&
\multicolumn{2}{c}{
  Does the review talk about the hotel’s location?
}

\end{tabular}

\vspace{6pt}

% =========================================================
% Activation regime legend (UNCHANGED, now at bottom)
% =========================================================
\begin{tikzpicture}
\tikzset{
  lgdot/.style={
    circle,
    minimum size=3.6pt,
    inner sep=0pt,
    draw,           % ensure a real path exists
    draw opacity=0  % but keep the outline invisible
  },
  legtxt/.style={font=\footnotesize, anchor=west}
}

\node[draw, rounded corners=2pt, inner sep=1pt] {%
  \begin{tikzpicture}
    \node[font=\footnotesize\bfseries, anchor=west] (ttl) {Activation regime};
    \matrix[matrix of nodes,
            below=2pt of ttl,
            column sep=14pt, row sep=1pt,
            nodes={legtxt}] {
      |[lgdot, fill=mplC1]| {} & Low--Low
      & |[lgdot, fill=mplC0]| {} & Low--High \\
      |[lgdot, fill=mplC3]| {} & High--Low
      & |[lgdot, fill=mplC2]| {} & High--High \\
    };
  \end{tikzpicture}%
};



\end{tikzpicture}

\caption{
Projection of hotel reviews onto the \emph{location} and \emph{staff} concept axes
for six scoring methods. Dashed lines indicate the $0.5$ thresholds defining the
four activation regimes.
}
\label{fig:hotel_multiplot}
\end{figure}


==> figures/fig_hotel_2x2_save.tex <==
\usetikzlibrary{matrix,positioning}

\begin{figure}[!t]
\centering
\footnotesize

\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.0}

\begin{tabular}{c c c}

% -------- First row --------
\parbox[c][0.55\linewidth][t]{1.8em}{%
  \vspace*{2cm}
  \rotatebox{90}{Does the review talk about hotel staff?}
}
&
\begin{subfigure}[t]{0.44\linewidth}
  \centering
  \includegraphics[width=\linewidth, trim={6pt 6pt 6pt 6pt},clip]{figures/hotel_tfidf.pdf}
  \caption{Sparse Lexical}
\end{subfigure}
&
\begin{subfigure}[t]{0.44\linewidth}
  \centering
  \includegraphics[width=\linewidth, trim={6pt 6pt 6pt 6pt},clip]{figures/hotel_cosine.pdf}
  \caption{Dense Neural}
\end{subfigure}
\\[-40pt]

% -------- Second row --------
&
\begin{subfigure}[t]{0.44\linewidth}
  \centering
  \includegraphics[width=\linewidth, trim={6pt 6pt 6pt 6pt},clip]{figures/hotel_direct_rating.pdf}
  \caption{Direct Rating}
\end{subfigure}
&
\begin{subfigure}[t]{0.44\linewidth}
  \centering
  \includegraphics[width=\linewidth, trim={6pt 6pt 6pt 6pt},clip]{figures/hotel_zero_shot.pdf}
  \caption{Probabilistic Zero-Shot}
\end{subfigure}
\\[20pt]

% -------- Third row --------
&
\begin{subfigure}[t]{0.44\linewidth}
  \centering
  \includegraphics[width=\linewidth, trim={6pt 6pt 6pt 6pt},clip]{figures/hotel_explanation_marginalized.pdf}
  \caption{Explanation-Marginalized}
\end{subfigure}
&
% -------- Legend replaces removed plot --------
\begin{minipage}[t]{0.44\linewidth}
  \vspace{-95pt}
  \hspace{11pt}
  \begin{tikzpicture}[baseline]
    \tikzset{
      lgdot/.style={circle, inner sep=0pt, minimum size=3.2pt, draw=none},
      legtxt/.style={font=\footnotesize, anchor=west}
    }

    \node[draw, rounded corners=2pt, inner sep=3pt] (box) {%
      \begin{tikzpicture}
        % Title (separate from the matrix)
        \node[font=\footnotesize\bfseries, anchor=west] (ttl) {Activation regime};

        % Items below title
        \matrix[matrix of nodes,
                below=3pt of ttl,
                column sep=8pt, row sep=0pt,
                nodes={legtxt}] (leg) {
          |[lgdot, fill=mplC1]| {} & Low--Low  \\
          |[lgdot, fill=mplC0]| {} & Low--High \\
          |[lgdot, fill=mplC3]| {} & High--Low   \\
          |[lgdot, fill=mplC2]| {} & High--High  \\
        };
      \end{tikzpicture}%
    };
  \end{tikzpicture}
\end{minipage}

\\[20pt]

% -------- X-axis label --------
&
\multicolumn{2}{c}{
  Does the review talk about the hotel’s location?
}

\end{tabular}

\caption{
Projection of hotel reviews onto the \emph{location} and \emph{staff} concept axes
for five scoring methods. Dashed lines indicate the $0.5$ thresholds defining the
four activation regimes.
}
\label{fig:hotel_multiplot}
\end{figure}


==> figures/surrogate_tree_old.tex <==
\begin{figure}[!t]
\centering
 
\begin{tikzpicture}[
    font=\footnotesize,
>=Latex,
    level distance=14mm,
    level 1/.style={sibling distance=42mm},
    level 2/.style={sibling distance=20mm},
    level 3/.style={sibling distance=9mm},
    every node/.style={draw, rounded corners=3pt, align=center, inner sep=3pt, font=\scriptsize},
    split/.style={fill=gray!10, text width=1.7cm},
    leaf/.style={fill=gray!5, text width=0.6cm, font=\scriptsize\bfseries},
    edge from parent/.style={draw, -Latex}
]
 
% -------- Header --------
\node[draw=none, fill=none, font=\footnotesize] (hdr)
{All internal nodes test: \emph{``Is this text about \texttt{<concept>}?''}};
 
% ---------------- Root ----------------
\node[split, below=4mm of hdr] (root) {
  \texttt{literacy-in-}\\
  \texttt{science}\\
  $\le 0.044$
}
% -------- Level 1 --------
child { node[split] {
\texttt{figurative-}\\
\texttt{language}\\
$\le 0.012$
}
    % -------- Level 2 (left subtree) --------
    child { node[split] {
    \texttt{economics}\\
    $\le 0.003$
    }
        % -------- Leaves --------
        child { node[leaf] {\textbf{Nat.}} }
        child { node[leaf] {\textbf{Soc.}} }
    }
    child { node[split] {
    \texttt{punctuation}\\
    $\le 0.075$
    }
        child { node[leaf] {\textbf{Lang.}} }
        child { node[leaf] {\textbf{Nat.}} }
    }
}
% -------- Level 1 (right subtree) --------
child { node[split] {
\texttt{word-study}\\
$\le 0.105$
}
    child { node[split] {
    \texttt{economics}\\
    $\le 0.298$
    }
        child { node[leaf] {\textbf{Nat.}} }
        child { node[leaf] {\textbf{Soc.}} }
    }
    child { node[split] {
    \texttt{literacy-in-}\\
    \texttt{science}\\
    $\le 0.733$
    }
        child { node[leaf] {\textbf{Lang.}} }
        child { node[leaf] {\textbf{Nat.}} }
    }
};

% ---- Manual Yes/No label near top-left edge ----
\node[
  draw,
  rounded corners=2pt,
  fill=white,
  inner sep=1.2pt,
  font=\scriptsize
] at ([xshift=-13.5mm,yshift=-5.5mm]root) {Yes};

\node[
  draw,
  rounded corners=2pt,
  fill=white,
  inner sep=1.2pt,
  font=\scriptsize
] at ([xshift=13.5mm,yshift=-5.5mm]root) {No};
 
\end{tikzpicture}
 
\caption{
Schematic decision-tree surrogate (three split levels) operating on zero-shot
concept activations. Each internal node thresholds the activation score for a
human-defined requirement, and each leaf outputs the predicted ScienceQA
subject (\textbf{Nat.} = Natural science, \textbf{Soc.} = Social science,
\textbf{Lang.} = Language science).
}
 
\label{fig:surrogate-decision-tree}
\end{figure}

==> tables/surrogate_examples_1.tex <==
\begin{table}[!t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{p{0.14\linewidth} p{0.80\linewidth}}
\toprule
\textbf{Class} & \textbf{Illustrative surrogate explanation} \\
\midrule

\textbf{Language science} &
\textbf{Text:} Which word would you find on a dictionary page with the following guide words?
tea -- triangle \\
& \textbf{True label:} Language science \\
& \textbf{Decision path:} \\
& ``Is this text about \ldots\ \\
& \texttt{literacy-in-science}? $s = 0.005 \le \tau = 0.044$ \\
& \quad$\rightarrow$ \texttt{figurative-language}? $s = 0.023 > \tau = 0.012$ \\
& \quad\quad$\rightarrow$ \texttt{punctuation}? $s = 0.010 \le \tau = 0.075$ \\
& \quad\quad\quad$\Rightarrow$ \textbf{Predicted: Language science} \\


\midrule

\textbf{Natural science} &
\textbf{Text:} Which type of relationship is formed when an epiphytic orchid grows on a tree branch in the canopy? \\
& \textbf{True label:} Natural science \\
& \textbf{Decision path:} \\
& ``Is this text about \ldots\ \\
& \texttt{literacy-in-science}? $s = 0.995 > \tau = 0.044$ \\
& \quad$\rightarrow$ \texttt{word-study}? $s = 0.001 \le \tau = 0.105$ \\
& \quad\quad$\rightarrow$ \texttt{economics}? $s = 0.000 \le \tau = 0.298$ \\
& \quad\quad\quad$\Rightarrow$ \textbf{Predicted: Natural science} \\


\midrule

\textbf{Social science} &
\textbf{Text:} Is a lamp a good or a service? \\
& \textbf{True label:} Social science \\
& \textbf{Decision path:} \\
& ``Is this text about \ldots\ \\
& \texttt{literacy-in-science}? $s = 0.077 > \tau = 0.044$ \\
& \quad$\rightarrow$ \texttt{word-study}? $s = 0.005 \le \tau = 0.105$ \\
& \quad\quad$\rightarrow$ \texttt{economics}? $s = 0.987 > \tau = 0.298$ \\
& \quad\quad\quad$\Rightarrow$ \textbf{Predicted: Social science} \\

\bottomrule
\end{tabular}
\caption{
Illustrative surrogate explanations produced by the decision tree.
For each subject, we report one test example together with the sequence
of requirement-based rules followed by the surrogate model.
At each internal node, $s(x,c)$ denotes the zero-shot alignment score
between text $x$ and concept $c$, and $\tau$ denotes the learned decision
threshold used by the surrogate.
}

\label{tab:surrogate-examples}
\end{table}

